MedPromptX: Grounded Multimodal Prompting for Chest X-ray Diagnosis

Chest X-ray images are commonly used for predicting acute and chronic cardiopulmonary conditions, but efforts to integrate them with structured clinical data face challenges due to incomplete electronic health records (EHR). This paper introduces MedPromptX, the first clinical decision support system that integrates multimodal large language models (MLLMs), few-shot prompting (FP) and visual grounding (VG) to combine imagery with EHR data for chest X-ray diagnosis. A pre-trained MLLM is utilized to complement the missing EHR information, providing a comprehensive understanding of patients' medical history. Additionally, FP reduces the necessity for extensive training of MLLMs while effectively tackling the issue of hallucination. Nevertheless, the process of determining the optimal number of few-shot examples and selecting high-quality candidates can be burdensome, yet it profoundly influences model performance. Hence, we propose a new technique that dynamically refines few-shot data for real-time adjustment to new patient scenarios. Moreover, VG narrows the search area in X-ray images, thereby enhancing the identification of abnormalities. We also release MedPromptX-VQA, a new in-context visual question answering dataset encompassing interleaved images and EHR data derived from MIMIC-IV and MIMIC-CXR-JPG databases. Results demonstrate the SOTA performance of MedPromptX, achieving an 11% improvement in F1-score compared to the baselines. Code and data are publicly available on https://github.com/BioMedIA-MBZUAI/MedPromptX.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/ablation_dino.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Performance analysis of VG. When VG is activated, the model processes images with contextual grounding. Conversely, when VG is deactivated, the model ingests original images.}
\label{tab:ablation_dino}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{@{}c|cccc@{}}
\toprule
\rowcolor[HTML]{D9D9D9} 
\textbf{VG   Setting} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Accuracy} \\ \midrule
VG Disabled           & 0.708              & \textbf{0.581}  & 0.658             & 0.659             \\
VG Enabled            & \textbf{0.773}              & 0.565           & \textbf{0.686}    & \textbf{0.689}    \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/ablation_dps.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Performance analysis of DPS. Without DPS, candidate prompts in the 6-shot setting are randomly ordered. In contrast, with DPS, the ordering is determined by cosine similarity scores between the embeddings of each candidate and the test prompt, potentially reducing the number of candidates per record given a threshold.}
\label{tab:ablation_dps}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{@{}c|cccc@{}}
\toprule
\rowcolor[HTML]{D9D9D9} 
\textbf{DPS   Setting} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Accuracy} \\ \midrule
DPS Disabled           & 0.520              & 0.379           & 0.486             & 0.500             \\
DPS Enabled            & \textbf{0.773}     & \textbf{0.565}  & \textbf{0.686}    & \textbf{0.689}    \\ \bottomrule
\end{tabular}%
}
\end{table}
